PVNAS: 3D Neural Architecture Search with Point-Voxel Convolution

3D neural networks are widely used in real-world applications (e.g., AR/VR headsets, self-driving cars). They are required to be fast and accurate; however, limited hardware resources on edge devices make these requirements rather challenging. Previous work processes 3D data using either voxel-based or point-based neural networks, but both types of 3D models are not hardware-efficient due to the large memory footprint and random memory access. In this paper, we study 3D deep learning from the efficiency perspective. We first systematically analyze the bottlenecks of previous 3D methods. We then combine the best from point-based and voxel-based models together and propose a novel hardware-efficient 3D primitive, Point-Voxel Convolution (PVConv). We further enhance this primitive with the sparse convolution to make it more effective in processing large (outdoor) scenes. Based on our designed 3D primitive, we introduce 3D Neural Architecture Search (3D-NAS) to explore the best 3D network architecture given a resource constraint. We evaluate our proposed method on six representative benchmark datasets, achieving state-of-the-art performance with 1.8-23.7x measured speedup. Furthermore, our method has been deployed to the autonomous racing vehicle of MIT Driverless, achieving larger detection range, higher accuracy and lower latency.

==> figures/results/partnet/visualizations.tex <==
\begin{figure*}[!t]
\centering
\begin{subfigure}[b]{\linewidth}
    \centering
    %\includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/0a.png}
    \includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/1a.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/2a.png}
    \includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/3a.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/4a.png}
    \includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/5a.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/6a.png}
    \includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/7a.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/8a.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/9a.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/10a.png}
    \includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/11a.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/12a.png}
    \includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/13a.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/14a.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/15a.png}
    \includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/16a.png}
    \includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/17a.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/18a.png}
    \caption{Predictions from PVNAS (4.3ms on GTX1080Ti).}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
    \centering
    %\includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/0b.png}
    \includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/1b.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/2b.png}
    \includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/3b.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/4b.png}
    \includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/5b.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/6b.png}
    \includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/7b.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/8b.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/9b.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/10b.png}
    \includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/11b.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/12b.png}
    \includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/13b.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/14b.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/15b.png}
    \includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/16b.png}
    \includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/17b.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/partnet/visualizations/18b.png}
    \caption{Ground truth segmentation.}
\end{subfigure}
\caption{PVNAS efficiently generates high quality fine-grained part segmentation results on PartNet~\cite{mo2019partnet}.}
\label{fig:exp:partnet:visualizations}
\end{figure*}


==> figures/results/shapenet/tradeoffs.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/exp/shapenet/tradeoffs/a}
        \caption{Trade-off: mean IoU \vs GPU latency}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/exp/shapenet/tradeoffs/b}
        \caption{Trade-off: mean IoU \vs GPU memory}
    \end{subfigure}
    \caption{PVCNN achieves a better trade-off between accuracy and efficiency than the point-based and voxel-based baselines on ShapeNet Part.}
    \label{fig:exp:shapenet:tradeoffs}
\end{figure*}


==> figures/results/shapenet/visualizations.tex <==
\begin{figure*}[!t]
\centering
\begin{subfigure}[b]{\linewidth}
    \centering
    \includegraphics[width=0.115\linewidth]{figures/exp/shapenet/visualizations/0a.png}
    \includegraphics[width=0.115\linewidth]{figures/exp/shapenet/visualizations/1a.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/shapenet/visualizations/2a.png}
    \includegraphics[width=0.115\linewidth]{figures/exp/shapenet/visualizations/3a.png}
    \includegraphics[width=0.115\linewidth]{figures/exp/shapenet/visualizations/4a.png}
    \includegraphics[width=0.115\linewidth]{figures/exp/shapenet/visualizations/5a.png}
    \includegraphics[width=0.115\linewidth]{figures/exp/shapenet/visualizations/6a.png}
    \includegraphics[width=0.115\linewidth]{figures/exp/shapenet/visualizations/7a.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/shapenet/visualizations/8a.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/shapenet/visualizations/9a.png}
    \includegraphics[width=0.115\linewidth]{figures/exp/shapenet/visualizations/10a.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/shapenet/visualizations/11a.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/shapenet/visualizations/12a.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/shapenet/visualizations/13a.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/shapenet/visualizations/14a.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/shapenet/visualizations/15a.png}
    \caption{Predictions from PVCNN (0.25$\times$ C).}
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
    \centering
    \includegraphics[width=0.115\linewidth]{figures/exp/shapenet/visualizations/0b.png}
    \includegraphics[width=0.115\linewidth]{figures/exp/shapenet/visualizations/1b.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/shapenet/visualizations/2b.png}
    \includegraphics[width=0.115\linewidth]{figures/exp/shapenet/visualizations/3b.png}
    \includegraphics[width=0.115\linewidth]{figures/exp/shapenet/visualizations/4b.png}
    \includegraphics[width=0.115\linewidth]{figures/exp/shapenet/visualizations/5b.png}
    \includegraphics[width=0.115\linewidth]{figures/exp/shapenet/visualizations/6b.png}
    \includegraphics[width=0.115\linewidth]{figures/exp/shapenet/visualizations/7b.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/shapenet/visualizations/8b.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/shapenet/visualizations/9b.png}
    \includegraphics[width=0.115\linewidth]{figures/exp/shapenet/visualizations/10b.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/shapenet/visualizations/11b.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/shapenet/visualizations/12b.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/shapenet/visualizations/13b.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/shapenet/visualizations/14b.png}
    %\includegraphics[width=0.115\linewidth]{figures/exp/shapenet/visualizations/15b.png}
    \caption{Ground truth segmentation.}
\end{subfigure}
\caption{Qualitative results of PVCNN (0.25$\times$ C) on ShapeNet~\cite{chang2015shapenet}.}
\label{fig:exp:shapenet:visualizations}
\end{figure*}


==> tables/taxonomy.tex <==
\begin{table}[t]
\caption{{Family of Point-Voxel Convolution}}
\label{tab:intro:taxonomy}
\renewcommand*{\arraystretch}{1.1}
\centering
\scalebox{0.75}{
\setlength{\columnsep}{1px}
\begin{tabular}{ccc}
\toprule
{\textbf{Name}} & {\textbf{Meaning}} & {\textbf{Suitable For}} \\
\midrule
{PVConv} & {Point-Voxel Convolution} & \multirow{6}{*}{\shortstack[c]{{Objects / Indoor Scans}\\ {(size $\approx$ 1.5m$\times$1.5m$\times$1.5m)}}} \\
\cline{1-2}\\[-8pt]
\multirow{2}{*}{{PVCNN}} & \multirow{2}{*}{\shortstack[c]{{Manually-Designed CNN}\\ {with PVConv}}} \\
\\
\cline{1-2}\\[-8pt]
\multirow{2}{*}{{PVNAS}} & \multirow{2}{*}{\shortstack[c]{{Automatically-Designed CNN}\\ {with PVConv}}} \\
\\
\midrule\midrule
{SPVConv} & {Sparse Point-Voxel Convolution} & \multirow{6}{*}{\shortstack[c]{{Large Outdoor Scenes}\\ {(size $\gg$ 1.5m$\times$1.5m$\times$1.5m)}}} \\
\cline{1-2}\\[-8pt]
\multirow{2}{*}{{SPVCNN}}   & \multirow{2}{*}{\shortstack[c]{{Manually-Designed CNN}\\ {with SPVConv}}} \\
\\
\cline{1-2}\\[-8pt]
\multirow{2}{*}{{SPVNAS}}   & \multirow{2}{*}{\shortstack[c]{{Automatically-Designed CNN}\\ {with SPVConv}}} \\
\\
\bottomrule
\end{tabular}
}
\end{table}
